Pseudorandom Isometries

We introduce a new notion called ${\cal Q}$-secure pseudorandom isometries (PRI). A pseudorandom isometry is an efficient quantum circuit that maps an $n$-qubit state to an $(n+m)$-qubit state in an isometric manner. In terms of security, we require that the output of a $q$-fold PRI on $\rho$, for $ \rho \in {\cal Q}$, for any polynomial $q$, should be computationally indistinguishable from the output of a $q$-fold Haar isometry on $\rho$. By fine-tuning ${\cal Q}$, we recover many existing notions of pseudorandomness. We present a construction of PRIs and assuming post-quantum one-way functions, we prove the security of ${\cal Q}$-secure pseudorandom isometries (PRI) for different interesting settings of ${\cal Q}$. We also demonstrate many cryptographic applications of PRIs, including, length extension theorems for quantum pseudorandomness notions, message authentication schemes for quantum states, multi-copy secure public and private encryption schemes, and succinct quantum commitments.

==> construction/haar_type.tex <==
\subsubsection{Security against Haar inputs}
In this section, we prove security against queries which are sampled i.i.d. from the Haar measure. In particular, we show the following theorem:
\begin{theorem}
\label{lem:haar_proof}
    Let $n,m,s,t = \poly(\secparam)$ and $\qclass_{n,q,\ell,\secparam}^{({\sf Haar})}$ be as defined in~\Cref{sec:defs} then, assuming the existence of post-quantum one-way functions, the construction of $\pri$ given in \Cref{fig:prp_prs} is $\qclass_{\mathsf{Haar}_{s,t}}$-secure. 
\end{theorem}

\noindent To prove this we first note that $$\E_{\ket{\vartheta_1},\cdots,\ket{\vartheta_s}\leftarrow\Haar_{n}}\left[\bigotimes_{i=1}^{s} \ketbra{\vartheta_i}{\vartheta_i}^{\otimes 2t}\right] = \E_{T_1,\cdots,T_s}\left[\bigotimes_{i=1}^{s} \ketbra{\type_{T_i}}{\type_{T_i}}\right],$$
where each $T_i$ is an i.i.d. sampled type containing $2t$ elements. We know that with overwhelming probability this lies in $\tuni{n}{s}{2t}$. Note that our construction is only acting on a half of each of the type states and not the complete states. Hence, if we prove security against queries from $\tuni{n}{s}{2t}$ with the construction being applied to only one half of each of the type states, we would get security for i.i.d. sampled Haar queries as required. In particular, we prove the following:
\begin{lemma}
\label{lem:tuni_info}
    Let $n,m,s,t = \poly(\secparam)$ and let $(T_1,\cdots,T_s)\in\tuni{n}{s}{2t}$. Let $G_{(f,\pi)}$ is as defined in \Cref{fig:info_prp_prs}. Let 
    $$\rho:= \E_{(f,\pi)\leftarrow(\mathcal{F}_{n+m},S_{n+m})} \bigotimes_{i=1}^{s} \left(\left(I_{nt}\otimes G_{(f,\pi)^{\otimes t}}\right)\ketbra{\type_{T_i}}{\type_{T_i}}\left(I_{nt}\otimes G_{(f,\pi)^{\otimes t}}\right)^{\dagger}\right),$$
    and $$\sigma:= \E_{\substack{(\overline{T}_1,\cdots,\overline{T}_s)\subset (T_1,\cdots,T_s)\\ \forall i\in [s], \hamming(\overline{T}_i)=t\\
    (\hat{T_1},\cdots,\hat{T_1})\leftarrow\tuni{n+m}{s}{t}}}\left(\ketbra{\type_{\overline{T}_i}}{\type_{\overline{T}_i}}\otimes\ketbra{\type_{\hat{T}_i}}{\type_{\hat{T}_i}}\right).$$
    Then $\TD(\rho,\sigma)=O(st^2/2^{m})$.
\end{lemma}
\begin{proof}[Proof sketch]
    We know from \Cref{lem:type_struc}, $\bigotimes_{i=1}^{s} \ketbra{\type_{T_i}}{\type_{T_i}}$ can be written as a sum over $\vec{x_i}\in T_i$, $\sigma_i\in S_{2t}$, $\bigotimes_{i=1}^{s} \ketbra{\vec{x_i}}{\sigma_i(\vec{x_i})}$. 
    Let each $\vec{x_i}$ (containing $2t$ elements) is a concatenation of $\vec{c_i}$ and $\vec{d_i}$ (where each contains $t$ elements). Note that, all elements of $\vec{x_i}$ are distinct, hence $\vec{c_i}$ and $\vec{d_i}$ also contain distinct elements. Notice that if any of the $\sigma_i$'s maps any of the first $t$ elements to the last $t$ elements, then by \Cref{lem:outer_comp_query}, we get $0$. Hence, we get that each $\sigma_i$ can be written as a combination $\sigma^1_i\in S_t$ and $\sigma^2_i\in S_t$ where $\sigma^1_i$ is applied to the first $t$ elements of $\vec{x_i}$ and $\sigma^2_i$ is applied to the last $t$ elements of $\vec{x_i}$. Hence, we get that the input is just of the form $\bigotimes_{i=1}^{s} \ketbra{\vec{c_i}}{\sigma^1_i(\vec{c_i})}\otimes\ketbra{\vec{d_i}}{\sigma^2_i(\vec{d_i})}$, with the construction being applied to the second half of each state. Notice that summing over all $\sigma^1_i,\sigma^2_i$, there are type states too. We know that the effect of the construction on the second half is very close to $\rho_{\unique}$ by \Cref{lem:tdis_info}. Hence, it gets unentangled from the first half and we get the desired result.
\end{proof}
\ifllncs
\noindent The proof of~\Cref{lem:tuni_info} can be found in~\Cref{app:closeness_to_rho_uni}. 
\else
\input{construction_proofs/tuni_info_proof}
\fi
\noindent Interestingly, \Cref{lem:tuni_info} implies that our construction is secure against a specific 
\emph{entangled} queries --- in $\ket{\type_{T_i}}$, adversary's registers and the registers acted on by the PRI are entangled. Using this, we prove the following for Haar states.
\begin{lemma}
    \label{lem:haar_info}
    Let $n,m,s,t = \poly(\secparam)$. Let $G_{(f,\pi)}$ be as defined in \Cref{fig:info_prp_prs}. Let 
    $$\rho:= \E_{(f,\pi)\leftarrow(\mathcal{F}_{n+m},S_{n+m})} \bigotimes_{i=1}^{s} \left(\E_{\ket{\vartheta_i}\leftarrow \Haar_{n}} \ketbra{\vartheta_i}{\vartheta_i}^{\otimes t} \otimes \left(G_{(f,\pi)}\ketbra{\vartheta_i}{\vartheta_i} G_{(f,\pi)}^{\dagger}\right)^{\otimes t}\right)$$ and let 
    $$\sigma := \E_{\substack{(T_1,\cdots,T_s)\leftarrow \tuni{n+m}{s}{t}\\ (\overline{T}_1,\cdots,\overline{T}_s)\leftarrow \tuni{n}{s}{t}}} \bigotimes_{i=1}^{s} \left( \left(\ketbra{\type_{\overline{T}_i}}{\type_{\overline{T}_i}}\right)\otimes \left(\ketbra{\type_{T_i}}{\type_{T_i}}\right) \right). $$ 
    Then $$\TD(\rho,\sigma) = O(s^2t^2/2^n+st^2/2^m).$$
\end{lemma}
\begin{proof}[Proof sketch]
    Note that we have $2t$ copies of $s$ i.i.d. sampled Haar states. Then by \Cref{fact:avg-haar-random}, this can be seen as i.i.d. sampling $T_1,...,T_s$ each over $2t$, elements. With very high probability, these $2st$ elements do not have any collisions, hence with very high probability $(T_1,...,T_s)$ is in $\mathcal{T}_{\unique}$. The security on each type in $\mathcal{T}_{\unique}$ is shown by \Cref{lem:tuni_info}.
\end{proof}
\ifllncs
\noindent The proof of~\Cref{lem:haar_info} can be found in~\Cref{app:closeness_to_rho_uni}.
\else
\input{construction_proofs/haar_info_proof}
\fi

\noindent Hence, combining \Cref{lem:haar_info} and \Cref{lem:comp_to_tuni}, we get the desired result. 

==> construction/single_input_type.tex <==
\subsubsection{Security against Multiple Copies of the Same Input}
\label{sec:security_multi_same}
In this section, we prove security against multiple copies of the same input. Formally, we prove the following,
 
\begin{theorem}
\label{lem:single_proof}
    Let $n,m,q = \poly(\secparam)$ and $\qclass^{(\single)}_{n,q,\ell,\secparam}$ be as defined in~\Cref{sec:defs} then, assuming the existence of post-quantum one-way functions, the construction of $\pri$ given in \Cref{fig:prp_prs} is $\qclass_{\mathsf{single}_{q}}$-secure.
\end{theorem}

Note that since $\ketbra{\phi}{\phi}^{\otimes q}$ is in the symmetric subspace, and type states form an orthogonal basis of the symmetric subspace, we can write $\ketbra{\phi}{\phi}^{\otimes q} = \sum_{T,T'}\alpha_{T,T'}\ketbra{\type_T}{\type_{T'}}$. Notice that, $\ketbra{\type_T}{\type_{T}}\in\qclass_{\distinct}$ for any type $T$. So, to find the action of $q$-fold $G_{(f,\pi)}$ on $\ketbra{\phi}{\phi}^{\otimes q}$, we just need to look at its action on $\ketbra{\type_T}{\type_{T'}}$ for $T\neq T'$. To do this, we analyze the output of the construction on $\ketbra{\vec{x}}{\vec{x'}}$ for $\type(\vec{x})\neq\type(\vec{x'})$.


\begin{lemma}
    \label{lem:outer_comp_query}
    Let $n,m\in\N$, $q\in\poly(\secparam)$, $\vec{x} = (x_1,\cdots,x_q)\in\{0,1\}^{nq}$, and $\vec{x'} = (x'_1,\cdots,x'_q)\in\{0,1\}^{nq}$. Let $\type(\vec{x})\neq\type(\vec{x'})$. Let $G_{(f,\pi)}$ be as defined in \Cref{fig:info_prp_prs}, then $$\E_{(f,\pi)\leftarrow(\mathcal{F}_{2^{n+m},p},S_{2^{n+m}})} \left[\left(G_{(f,\pi)}^{\otimes q}\right)\left(\bigotimes_{i=1}^{q}\ketbra{x_i}{x'_i}\right)\left(G_{(f,\pi)}^{\dagger}\right)^{\otimes q}\right]=0.$$
\end{lemma}
\begin{proof}[Proof sketch]
    We again see $G_{(f,\pi)}$ as $O_{\pi}O_{f}C_{\ket{+^m}}$. Acting on $\bigotimes_{i=1}^{q}\ketbra{x_i}{x'_i}$, applying $C_{\ket{+^m}}$ results in $\bigotimes_{i=1}^{q}\ketbra{x_i||a_i}{x'_i||a'_i}$ for each $a_i,a'_i\in\bit^m$. Applying $O_f$ gives us a leading coefficient of $\omega_p^{\sum_i (f(x_i||a_i)-f(x'_i||a'_i))}$ which always goes to zero when we take expectation over $f$ because $\sum_i (f(x_i||a_i)-f(x'_i||a'_i))\neq 0$ for all values of $a_i,a'_i$'s. Hence, we get that the resulting matrix is also zero.
\end{proof}
\ifllncs
\noindent The proof of~\Cref{lem:outer_comp_query} can be found in~\Cref{app:closeness_to_rho_uni}.
\else
\input{construction_proofs/comp_outer_query_proof}
\fi

\noindent A corollary of the above lemma is as follows,
\begin{corollary}
    \label{lem:type_outer}
    Let $n,m\in\N$, $q\in\poly(\secparam)$, $T,T'\in[q+1]^{2^{n}}$ with $T\neq T'$ and $\hamming(T) = \hamming(T') = q$. Let $G_{(f,\pi)}$ be as defined in \Cref{fig:info_prp_prs}, then $$\E_{(f,\pi)\leftarrow(\mathcal{F}_{2^{n+m},p},S_{2^{n+m}})} \left[\left(G_{(f,\pi)}^{\otimes q}\right)\ketbra{\type_{T}}{\type_{T'}}\left(G_{(f,\pi)}^{\dagger}\right)^{\otimes q}\right]=0.$$
\end{corollary}

\noindent Using the above, we get that the output of $q$-fold $G_{(f,\pi)}$ on  $\ketbra{\phi}{\phi}^{\otimes q}$, is close to $\rho_{\unique}$. Formally, we prove the following,
\begin{lemma}
    \label{lem:multicopy_info}
    Let $n,m,q=\poly(\secparam)$, $\ket{\phi}$ be any $n$ qubit pure state. Let $G_{(f,\pi)}$ be as defined in \Cref{fig:info_prp_prs}, let $$\rho = \E_{(f,\pi)\leftarrow(\mathcal{F}_{2^{n+m},p},S_{2^{n+m}})} \left[\left(G_{(f,\pi)}^{\otimes q}\right)\ketbra{\phi}{\phi}^{\otimes q}\left(G_{(f,\pi)}^{\dagger}\right)^{\otimes q}\right],$$
    and 
    $$\rho_{\unique} = \E_{(\overline{T}_1,\cdots,\overline{T}_q)\leftarrow \tuni{m+n}{1}{q}} \left[\ketbra{\type_{\overline{T}_i}}{\type_{\overline{T}_i}}\right].$$
    Then $\TD(\rho,\rho_{\unique}) = O(q^2/2^m)$.
\end{lemma}
\begin{proof}[Proof sketch]
    Since $\ketbra{\phi}{\phi}^{\otimes q}$ is in the symmetric subspace, we can write $\ketbra{\phi}{\phi}^{\otimes q} = \sum_{T,T'}\alpha_{T,T'}\ketbra{\type_T}{\type_{T'}}$. By \Cref{lem:type_outer}, the only terms remaining in this sum are when $T=T'$. The security on this is just implied by \Cref{lem:tdis_info}.
\end{proof}
\ifllncs
\noindent The proof of~\Cref{lem:multicopy_info} can be found in~\Cref{app:closeness_to_rho_uni}.
\else
\input{construction_proofs/multicopy_proof}
\fi
\noindent Combining \Cref{lem:multicopy_info} and \Cref{lem:comp_to_tuni}, we get the desired result. 

==> construction/type_distinct.tex <==
\subsubsection{Security against Distinct Types}
We define a class of state $$\qclass^{(\distinct)}_{{n,t,s,\ell,\secparam}}:= {\color{red}{\cal D}(\C^{2^{\ell'(\secparam)}})} \otimes\set{{\color{blue}\bigotimes_{i=1}^{s}\ketbra{\type_{T_i}}{\type_{T_i}}}:(T_1,\cdots,T_s)\in\tdis{n}{s}{t}}.$$
Next, we define the following class: 
$$\qclass^{(\distinct)}_{{n,q,\ell,\secparam}}:= \cup_{\substack{s,t\\\text{ such that } q=st}}\qclass^{(\distinct)}_{{n,t,s,\ell,\secparam}}.$$
In this section, we prove the security of the construction on $\qclass_{(\distinct)} := \set{\qclass^{(\distinct)}_{{n,q,\ell,\secparam}}}_{\secparam}$. In particular, we prove the following:

\begin{theorem}
\label{lem:tdis_proof}
    Let $n,m,q,\ell = \poly(\secparam)$ and $\qclass_{\distinct} $ be as defined above, then, assuming the existence of post-quantum one-way functions, the construction of $\pri$ given in \Cref{fig:prp_prs} is $\qclass_{\distinct}$-secure.
\end{theorem}

A straightforward corollary of the above theorem is that our construction is secure against computational basis state input. This is because for any $x\in\set{0,1}$, $\ket{x,\cdots,x}$ is a valid type state. Hence, we get the following:

\begin{corollary}
\label{lem:comp_proof}
    Let $n,m,q,\ell = \poly(\secparam)$ and $\qclass_{\comp}$ be as defined in \Cref{sec:defs}, then, assuming the existence of post-quantum one-way functions, the construction of $\pri$ given in \Cref{fig:prp_prs} is $\qclass_{\comp}$-secure.
\end{corollary}

To prove this, we show that the output of $G_{(f,\pi)}$ on any $\bigotimes_{i=1}^{s}\ketbra{\type_{T_i}}{\type_{T_i}}$ for $(T_1,\cdots,T_s)\in\tdis{n}{s}{t}$ is negligibly close to $\rho_{\mathsf{uni}}$.
\begin{lemma}
    \label{lem:tdis_info}
    Let $n,m,t,s = \poly(\secparam)$. Let $(T_1,\cdots,T_s)\in\tdis{n}{s}{t}$. 
    Let 
    $$\rho := \E_{(f,\pi)\leftarrow(\mathcal{F}_{2^{n+m},p},S_{2^{n+m}})}\left[\bigotimes_{i=1}^{s}G_{(f,\pi)}^{\otimes t}\ketbra{\type_{T_i}}{\type_{T_i}}(G_{(f,\pi)}^{\dagger})^{\otimes t}\right],$$
    and 
    $$\rho_{\unique} := \E_{(\overline{T}_1,\cdots,\overline{T}_s)\leftarrow \tuni{m+n}{s}{t}} \left[\bigotimes_{i=1}^{s} \ketbra{\type_{\overline{T}_i}}{\type_{\overline{T}_i}}\right].$$
    Then $\TD(\rho,\rho_{\unique}) = O(st^2/2^m)$.
\end{lemma}
\begin{proof}[Proof sketch]
    Observe that $\ketbra{\type_{T_1}}{\type_{T_1}}\otimes\cdots\otimes\ketbra{\type_{T_s}}{\type_{T_s}}$ can be seen as a convex sum over $\ketbra{\vec{x_1},\cdots,\vec{x_s}}{\vec{x'_1},\cdots,\vec{x'_s}}$ where $\vec{x_i},\vec{x'_i}\in T_i$. By \Cref{lem:type_struc}, this can equivalently be written as a sum over $\vec{x_i}\in T_i$, $\sigma_i\in S_t$, $\ketbra{\vec{x_1},\cdots,\vec{x_s}}{\sigma_1(\vec{x_1}),\cdots,\sigma_s(\vec{x'_s})}$. Applying $G_{(f,\pi)}$ can be seen as three operators, $C_{\ket{+^m}}$ which appends $\ket{+^m}$ to each entry, $O_f$ which maps $\ket{\vec{x_i}}$ to $\omega_p^{f(\vec{x_i})}\ket{\vec{x_i}}$ and $O_{\pi}$ which maps $\ket{\vec{x_i}}$ to $\ket{\vec{x_i}_{\pi}}$. Let us look at these effects one at a time. 
    \begin{enumerate}
        \item $C_{\ket{+^m}}$: We first apply to every register of the convex sum over $\ketbra{\vec{x_1},\cdots,\vec{x_s}}{\vec{x'_1},\cdots,\vec{x'_s}}$, this is equivalent to mapping each \newline $\ketbra{\vec{x_1},\cdots,\vec{x_s}}{\sigma_1(\vec{x_1}),\cdots,\sigma_s(\vec{x_s}})$ to a sum over  \newline $\ketbra{\vec{x_1}||\vec{a_1},\cdots,\vec{x_s}||\vec{a_s}}{\sigma_1(\vec{x_1})||\vec{a'_1},\cdots,\sigma_s(\vec{x_s})||\vec{a'_s}}$ for all $\vec{a_i},\vec{a'_i}\in\bit^{mt}$.
        \item $O_f$: When we apply $O_f$, we get a leading coefficient of $\omega_p^{f(\vec{x_i}||\vec{a_i})-f(\sigma_i(\vec{x_i})||\vec{a'_i})}$ on each term. Since $p>t$,\footnote{We will drop the subscript of $p_\secp$ and instead write $p$ for short.} taking expectation over $f$ would map this to zero unless $\vec{a'_i} = \sigma_i(\vec{a_i})$. Hence, the only terms left after this step are $\ketbra{\vec{x_1}||\vec{a_1},\cdots,\vec{x_s}||\vec{a_s}}{\sigma_1(\vec{x_1}||\vec{a_1}),\cdots,\sigma_s(\vec{x_s}||\vec{a_s})}$. 
        \item $O_{\pi}$: Notice that the state is a sum over all $(\vec{a_1},\cdots,\vec{a_s})$. With very high probability all elements of $(\vec{a_1},\cdots,\vec{a_s})$ are distinct. In this case, $\ketbra{\vec{x_1}||\vec{a_1},\cdots,\vec{x_s}||\vec{a_s}}{\sigma_1(\vec{x_1}||\vec{a_1}),\cdots,\sigma_s(\vec{x_s}||\vec{a_s})}$ has only distinct elements and applying $O_{\pi}$ maps it to random vectors with distinct elements. Taking sum over all $\sigma_i$, we get that this is equivalent to sampling from $\mathcal{T}_{\unique}$.
    \end{enumerate}
\end{proof}

% \noindent The proof of~\Cref{lem:tdis_info} can be found in~\Cref{app:closeness_to_rho_uni}.
\input{construction_proofs/type_distinct_proof}

Combining \Cref{lem:tdis_info} and \Cref{lem:comp_to_tuni}, we get the desired result.

==> haar_ortho.tex <==

\begin{proof}
    We start by analysing $$\rho = \E_{U\gets\overline{\Haar_{l}}} \left[\otimes_{i=1}^{s}\left(U^{\otimes t}\ketbra{x_i}{x_i}^{\otimes t}\left(U^{\dagger}\right)^{\otimes t}\right)\right].$$ 
    Note that by unitary invariance, we can write this state as  $$\rho = \E_{U\gets\overline{\Haar_{l}}} \left[\otimes_{i=1}^{s}\left(U^{\otimes t}\ketbra{i}{i}^{\otimes t}\left(U^{\dagger}\right)^{\otimes t}\right)\right].$$ 
    Since, $i$ is over $l$ bits but only needs $\log (s)$ bits to represent, hence, we can write $i$ over the first $\log (s)$ bits and $0^{l-\log (s)}$ in the rest of the qubits. Hence, 
    $$\rho = \E_{U\gets\overline{\Haar_{l}}} \left[\otimes_{i=1}^{s}\left(U^{\otimes t}\ketbra{i||0^{l-\log (s)}}{i||0^{l-\log (s)}}^{\otimes t}\left(U^{\dagger}\right)^{\otimes t}\right)\right].$$ 
    By unitary invariance of the Haar measure, we can  apply $(I\otimes H^{l-\log(s)})$, $O_f$, $O_{\pi}$. This is equivalent to applying the construction $G_{(f,\pi)}$ for $n=\log(s)$ and $m=l-\log(s)$. Hence, we can equivalently write this as \pnote{I'm not sure why we start talking about our construction here..}
    $$\rho = \E_{\substack{U\gets\overline{\Haar_{l}}\\ (f,\pi)}} \left[\otimes_{i=1}^{s}\left(UG_{(f,\pi)}\ketbra{i}{i}G_{(f,\pi)}^{\dagger} U^{\dagger}\right)^{\otimes t}\right].$$ 
    Using \Cref{lem:tdis_info}, we get that this is close to the following state with trace distance bounded by $O(s^2t^2/2^{l-\log(s)})$:
    $$\xi = \E_{U\gets\overline{\Haar_{l}}} \left[U^{\otimes st}\left(\rho_{\unique}\right)\left(U^{\dagger}\right)^{\otimes st}\right].$$ 
    Then by \Cref{lem:tuni_haar_dis}, we get that $\xi$ is $O(s^2t^2/2^{l})$ away from the following state,
    $$\sigma = \E_{U_1,\cdots,U_s\gets\overline{\Haar_{l}}} \left[\otimes_{i=1}^{s}\left(U_i^{\otimes t}\ketbra{0^l}{0^l}^{\otimes t}\left(U_i^{\dagger}\right)^{\otimes t}\right)\right].$$
    Hence, we get the desired distance of $O(s^2t^2/2^{l-\log(s)}) = O(s^3t^2/2^{l})$.
\end{proof}

==> temp-analysis.tex <==
\input{construction/comp_to_info}
\input{construction/invar_to_sec}
\input{construction/rho_uni}
\input{construction/closeness_to_rho_uni}
